Efficient Algorithms for Privately Releasing Marginals via Convex Relaxations

Consider a database of $n$ people, each represented by a bit-string of length $d$ corresponding to the setting of $d$ binary attributes. A $k$-way marginal query is specified by a subset $S$ of $k$ attributes, and a $|S|$-dimensional binary vector $\beta$ specifying their values. The result for this query is a count of the number of people in the database whose attribute vector restricted to $S$ agrees with $\beta$. Privately releasing approximate answers to a set of $k$-way marginal queries is one of the most important and well-motivated problems in differential privacy. Information theoretically, the error complexity of marginal queries is well-understood: the per-query additive error is known to be at least $\Omega(\min\{\sqrt{n},d^{\frac{k}{2}}\})$ and at most $\tilde{O}(\min\{\sqrt{n} d^{1/4},d^{\frac{k}{2}}\})$. However, no polynomial time algorithm with error complexity as low as the information theoretic upper bound is known for small $n$. In this work we present a polynomial time algorithm that, for any distribution on marginal queries, achieves average error at most $\tilde{O}(\sqrt{n} d^{\frac{\lceil k/2 \rceil}{4}})$. This error bound is as good as the best known information theoretic upper bounds for $k=2$. This bound is an improvement over previous work on efficiently releasing marginals when $k$ is small and when error $o(n)$ is desirable. Using private boosting we are also able to give nearly matching worst-case error bounds. Our algorithms are based on the geometric techniques of Nikolov, Talwar, and Zhang. The main new ingredients are convex relaxations and careful use of the Frank-Wolfe algorithm for constrained convex minimization. To design our relaxations, we rely on the Grothendieck inequality from functional analysis.

==> connection.tex <==
\newcommand{\Dee}{p}
\newcommand{\K}{K}
%\newcommand{\L}{\mathcal{L}}

\section{Connection to Refuting random $k$-XOR formulae}

In this section we argue that our bound on efficient approximation of the polytope $\K$ is unlikely to be improvable using the kind of techniques we employ. We do so by showing that approximating $\K$ when we measure the width under a different distribution would imply an algorithm for refuting random $k$-XOR formulae of low density.

Recall that the Gaussian width of the polytope $\K$ is defined as $\ex_{w \sim G}[\max_{v \in \K} \langle w, v\rangle] = \ex_{w \sim G}\|w\|_{\K^o}$. We next define a distribution $\Dee_p$ on $\{-1,0,1\}$ parameterized by a $p\in[0,1]$:
\begin{align*}
\Pr_{b \sim \Dee_p}[b=1] &= \frac{p}{2}\\
\Pr_{b \sim \Dee_p}[b=-1] &= \frac{p}{2}\\
\Pr_{b \sim \Dee_p}[b=0] &= 1-p\\
\end{align*}
Thus $\ex_{b \sim \Dee_p}[b]=0$ and $\ex_{b \sim \Dee_p}[b^2]=p$. Define the $\Dee_p$-width of $\K$ to be the expectation of the dual norm, when each $w_i$ is drawn independently from $\Dee_p$.

Recall that our polytope of choice $\K$ is the convex hull of the vectors $\{v^x \in \{-1,1\}^{d \choose k} :  x \in \{-1,1\}^d \mbox{ such that } v^x_S = \Pi_{i\in S} x_i\}$.
Note that each non-zero $w_S $ naturally corresponds to a constraint $ \Pi_{i\in S} x_i = w_S$. For a random $S$ and random sign, this gives us a random $k$-XOR constraint. Viewing the $\{-1,0,1\}$ vector $w$ as a subset of $k$-XOR clauses on $d$ variables, the dot product $\langle w,v^x\rangle$ counts the difference between the number of clauses that are satisfied by the assingment $x$ and the number of clauses that are not satisfied. Thus the dual norm $\|w\|_{\K^o}$ is exactly the advantage over random of the best assignment for the instance defined by $w$. Here we measure the advantage in absolute rather than relative terms.

Schoenebeck~\cite{Schoenebeck08} proves the following result:
%\begin{theorem}
%For any integer $k$ and any $\delta,\gamma>0$, there is a constant $\alpha$ such  that the following holds. Let $\phi$ be a random $k$-XOR instance over $d$ variables with $m=d^{\frac{k(1-2\gamma)}{2}}$. Then with probability $(1-o(1)$,
%\begin{itemize}
%\item The advantage of $\phi$ over random is at most $\delta\cdomt m$.
%\item The $\alpha d^{\gamma}$ level Lassere hierarchy permits a feasible solution.
%\end{itemize}
%\end{theorem}
\begin{theorem}
For any integer $k$ and any $\delta,\gamma>0$, there is a constant $\alpha$ such  that the following holds. Let $\phi$ be a random $k$-XOR instance over $d$ variables where each of $2{d \choose k}$ clauses occurs with probability $\frac{m}{2{d \choose k}}$, where $m=d^{\frac{k(1-2\gamma)}{2}}$. Then with probability $(1-o(1))$,
the $\alpha d^{\gamma}$ level Lassere hierarchy permits a feasible solution.
\end{theorem}

On the other hand, by a simple union bound argument, it follows that the advantage over random for a $\phi$ chosen at random, is at most $\sqrt{m d}$.
This translates to saying that for $p=\frac{m}{{d \choose k}}$,
\begin{itemize}
\item The $\Dee_p$ width of $\K$ is $\sqrt{md}$.
\item The $\Dee_p$ width of the $\alpha d^{\gamma}$- level Lassere relaxation of $\K$ is $(1-o(1))\frac{m}{2}$.
\end{itemize}

Thus a polynomial number of levels of Lassere do not approximate the $\Dee_p$-width of $\K$ better than a factor of $\sqrt{\frac{m}{d}} = d^{\frac{k(1-2\gamma)}{4} - \frac{1}{2}}$.

In particular, this implies that if one wants to find an $\L$ containing $\K$ such that $\K \subseteq \L \subseteq C\cdot \K$, then the $o(n^{\gamma})$-level Lasserre relaxation will not yield an $C$ better than $d^{\frac{k(1-2\gamma)}{4} - \frac{1}{2}}$.

Moreover, this suggests that approximating $\K$ better in the average
sense that we need would also require new techniques. The techniques
we used work also for $\Dee_p$ width using standard probabilistic arguments. Any approach to improving our bounds would require techniques that go not work for $\Dee_p$ width.





==> connectionnew.tex <==
\newcommand{\Dee}{\mathcal{D}}
\newcommand{\K}{\mathcal{K}}
%\newcommand{\L}{\mathcal{L}}

\section{Connection to Refuting random $k$-XOR formulae}

In this section we argue that our bound on efficient approximation of the polytope $\K$ is unlikely to be improvable using the kind of techniques we employ. We do so by showing that approximating $\K$ when we measure the width under a different distribution would imply an algorithm for refuting random $k$-XOR formulae of low density.

Recall that the Gaussian width of the polytope $\K$ is defined as $\ex_{w \sim G}[\max_{v \in \K} \langle w, v\rangle] = \ex_{w \sim G}\|w\|_{\K^o}$. We next define a distribution $\Dee_p$ on $\{-1,0,1\}$ parameterized by a $p\in[0,1]$:
\begin{align*}
\Pr_{b \sim \Dee_p}[b=1] &= \frac{p}{2}\\
\Pr_{b \sim \Dee_p}[b=-1] &= \frac{p}{2}\\
\Pr_{b \sim \Dee_p}[b=0] &= 1-p\\
\end{align*}
Thus $\ex_{b \sim \Dee_p}[b]=0$ and $\ex_{b \sim \Dee_p}[b^2]=p$. Define the $\Dee_p$-width of $\K$ to be the expectation of the dual norm, when each $w_i$ is drawn independently from $\Dee_p$.

Recall that our polytope of choice $\K$ is the convex hull of the vectors $\{v^x \in \{-1,1\}^{d \choose k} :  x \in \{-1,1\}^d \mbox{ such that } v^x_S = \Pi_{i\in S} x_i\}$.
Note that each non-zero $w_S $ naturally corresponds to a constraint $ \Pi_{i\in S} x_i = w_S$. For a random $S$ and random sign, this gives us a random $k$-XOR constraint. Viewing the $\{-1,0,1\}$ vector $w$ as a subset of $k$-XOR clauses on $d$ variables, the dot product $\langle w,v^x\rangle$ counts the difference between the number of clauses that are satisfied by the assingment $x$ and the number of clauses that are not satisfied. Thus the dual norm $\|w\|_{\K^o}$ is exactly the advantage over random of the best assignment for the instance defined by $w$. Here we measure the advantage in absolute rather than relative terms.

Schoenebeck~\cite{Schoenebeck08} proves the following result:
%\begin{theorem}
%For any integer $k$ and any $\delta,\gamma>0$, there is a constant $\alpha$ such  that the following holds. Let $\phi$ be a random $k$-XOR instance over $d$ variables with $m=d^{\frac{k(1-2\gamma)}{2}}$. Then with probability $(1-o(1)$,
%\begin{itemize}
%\item The advantage of $\phi$ over random is at most $\delta\cdomt m$.
%\item The $\alpha d^{\gamma}$ level Lassere hierarchy permits a feasible solution.
%\end{itemize}
%\end{theorem}
\begin{theorem}
For any integer $k$ and any $\delta,\gamma>0$, there is a constant $\alpha$ such  that the following holds. Let $\phi$ be a random $k$-XOR instance over $d$ variables where each of $2{d \choose k}$ clauses occurs with probability $\frac{m}{2{d \choose k}}$, where $m=d^{\frac{k(1-2\gamma)}{2}}$. Then with probability $(1-o(1))$,
the $\alpha d^{\gamma}$ level Lassere hierarchy permits a feasible solution.
\end{theorem}

On the other hand, by a simple union bound argument, it follows that the advantage over random for a $\phi$ chosen at random, is at most $\sqrt{m d}$.
This translates to saying that for $p=\frac{m}{{d \choose k}}$,
\begin{itemize}
\item The $\Dee_p$ width of $\K$ is $\sqrt{md}$.
\item The $\Dee_p$ width of the $\alpha d^{\gamma}$- level Lassere relaxation of $\K$ is $(1-o(1))\frac{m}{2}$.
\end{itemize}

Thus a polynomial number of levels of Lassere do not approximate the $\Dee_p$-width of $\K$ better than a factor of $\sqrt{\frac{m}{d}} = d^{\frac{k(1-2\gamma)}{4} - \frac{1}{2}}$.

In particular, this implies that if one wants to find an $\L$ containing $\K$ such that $\K \subseteq \L \subseteq C\cdot \K$, then the $o(n^{\gamma})$-level Lasserre relaxation will not yield an $C$ better than $d^{\frac{k(1-2\gamma)}{4} - \frac{1}{2}}$.

Moreover, this suggests that approximating $\K$ better in the average sense that we need would also require new techniques. The techniques we used work also for $\Dee_p$ width using known results from Random Matrix Theory(e.g.~\cite{TaoBook} Exercise 2.3.7 suffices). Any approach to improving our bounds would require techniques that go not work for $\Dee_p$ width.





==> spectral.tex <==
\section{Spectral Relaxation for Conjunctions}
